EvoChain: a Recovery Approach for Permissioned Blockchain Applications

Blockchain technology supports decentralized, consensus-driven data storage and processing, ensuring integrity and auditability. It is increasingly adopted for use cases with multiple stakeholders with shared ownership scenarios like digital identity and supply chain management. However, real-world deployments face challenges with mistakes and intrusions. This article presents EvoChain, a chaincode framework extension introducing controlled mutability for data redaction and recovery under time-limited or specific conditions. This mechanism allows corrections during a grace period before immutability takes effect. We validated our approach using WineTracker, a Hyperledger Fabric-based supply chain application. It enables some users to cancel unwanted operations while preserving the blockchain security and maintaining data consistency. Performance evaluations showed minimal overhead with functional benefits.

==> throughput_by_func_round.tex <==
\begin{figure}[!htb]
    \centering
    \small
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            symbolic x coords={createGrapes, sellGrapes, transformGrapes, cancelCreateGrapes},
            xtick=data,
            xlabel={Function},
            ylabel={Throughput (TPS)},
            legend entries={Round 1, Round 2, Round 3, Round 4, Round 5},
            legend style={at={(0.5,1.15)}, anchor=south, legend columns=3, font=\footnotesize},
            ymin=0, ymax=300,
            x tick label style={rotate=30,anchor=east, font=\small},
            width=0.65\textwidth,
            height=0.4\textwidth,
            enlarge x limits=0.18,
            bar width=8pt
        ]
        
        \addplot+[fill=blue!60] table[x=Name, y=Throughput] {Data/cancel1_evo.dat};
        \addplot+[fill=red!60] table[x=Name, y=Throughput] {Data/cancel2_evo.dat};
        \addplot+[fill=green!60] table[x=Name, y=Throughput] {Data/cancel3_evo.dat};
        \addplot+[fill=orange!60] table[x=Name, y=Throughput] {Data/cancel4_evo.dat};
        \addplot+[fill=purple!60] table[x=Name, y=Throughput] {Data/cancel5_evo.dat};

        \end{axis}
    \end{tikzpicture}
    \caption{Throughput (TPS) by Function and Test Round for TC2 Scenario}
    \label{fig:tc2_throughput_round}
\end{figure}


\begin{comment}
    
\begin{figure}[!htb]
  \centering
  \small
  \begin{tikzpicture}
    \begin{axis}[
      ybar,
      symbolic x coords={createGrapes, sellGrapes, transformGrapes, cancelCreateGrapes},
      xtick=data,
      xlabel={Function},
      ylabel={Throughput(TPS)},
      legend entries={Round 1, Round 2, Round 3, Round 4, Round 5},
      legend pos=north west,
        legend style={at={(0.5,1.05)}, anchor=south, legend columns=2}, 
      ymin=0, ymax=300,  
      x tick label style={rotate=30,anchor=east},
      width=0.60\textwidth,
      height=0.35\textwidth,  
      enlarge x limits=0.18,
    ]
    
    \addplot+[fill=blue!40, bar width=7pt] table[x=Name, y=Throughput] {Data/cancel1_evo.dat};
    \addplot+[fill=red!40, bar width=7pt] table[x=Name, y=Throughput] {Data/cancel2_evo.dat};
    \addplot+[fill=green!40, bar width=7pt] table[x=Name, y=Throughput] {Data/cancel3_evo.dat};
    \addplot+[fill=orange!40, bar width=7pt] table[x=Name, y=Throughput] {Data/cancel4_evo.dat};
    \addplot+[fill=purple!40, bar width=7pt] table[x=Name, y=Throughput] {Data/cancel5_evo.dat};

    \end{axis}
  \end{tikzpicture}
  \caption{TC2 Throughput by Function and Round}
  \label{fig:tc2_throughput_round}
\end{figure}
\end{comment}
